Graph Elicitation for Guiding Multi-Step Reasoning in Large Language Models

Chain-of-Thought (CoT) prompting along with sub-question generation and answering has enhanced multi-step reasoning capabilities of Large Language Models (LLMs). However, prompting the LLMs to directly generate sub-questions is suboptimal since they sometimes generate redundant or irrelevant questions. To deal with them, we propose a GE-Reasoning method, which directs LLMs to generate proper sub-questions and corresponding answers. Concretely, given an input question, we first prompt the LLM to generate knowledge triplets, forming a graph representation of the question. Unlike conventional knowledge triplets, our approach allows variables as head or tail entities, effectively representing a question as knowledge triplets. Second, for each triplet, the LLM generates a corresponding sub-question and answer along with using knowledge retrieval. If the prediction confidence exceeds a threshold, the sub-question and prediction are incorporated into the prompt for subsequent processing. This approach encourages that sub-questions are grounded in the extracted knowledge triplets, reducing redundancy and irrelevance. Our experiments demonstrate that our approach outperforms previous CoT prompting methods and their variants on multi-hop question answering benchmark datasets.

==> 3_methods/3_1_preliminaries.tex <==


In this section, we formulate CoT prompting method for question answering tasks. 
We use an Large Language Model~(LLM), denoted by $p_{\theta}\left(\boldsymbol{x} \right)$, to predict an answer of the question in the autoregressive manner. 
It can be formulated as $p_{\theta}\left(\boldsymbol{x} \right) = \Pi_{i=1}^n p_{\theta}\left(\boldsymbol{x}_i | \boldsymbol{x}_{<i} \right)$, where $\boldsymbol{x}_{<i}$ is the token sequence before the $i$-th token.

\subsection{Chain-of-Thought (CoT) prompting}%~\cite{wei2022chain}}
% \paragraph{Chain-of-Thought (CoT) prompting~\cite{wei2022chain}.}
CoT prompting is proposed to deal with complex problems requiring intermediate reasoning steps.
The idea is to predict the answer $\boldsymbol{y}$ with the intermediate reasoning steps $\mathcal{Z} = \boldsymbol{z}^{(1)}, \dots \boldsymbol{z}^{(m)}$, where each rationale $\boldsymbol{z}^{(j)}$ is an intermediate step for the reasoning and $m$ denotes the number of reasoning steps.
The rationale $\boldsymbol{z}^{(j)} \sim p_{\theta}\left(\boldsymbol{z}^{(j)}|\mathcal{E}, \boldsymbol{x}, \boldsymbol{z}^{(<j)}\right)$ is sampled sequentially until reaching the answer.
In sum, predicting an answer with CoT prompting can be formulated as
\begin{equation}
\begin{split}
    &\hat{\boldsymbol{y}} =  \underset{\boldsymbol{y}}{\arg\!\max}\ \ p_{\theta}\left(\boldsymbol{y} | \mathcal{E}, \boldsymbol{x}\right),\\
    &\mbox{where } p_{\theta}\left(\boldsymbol{y} | \mathcal{E}, \boldsymbol{x}\right)\\
    &=\int_{\mathcal{Z}}\ p_{\theta}\left(\boldsymbol{y} | \mathcal{E}, \boldsymbol{x}, \mathcal{Z}\right) p_{\theta}\left(\mathcal{Z} | \mathcal{E}, \boldsymbol{x}  \right),
\end{split}
\end{equation}
where $p_{\theta}\left(\mathcal{Z} | \mathcal{E}, \boldsymbol{x}  \right)=\prod_{j} p_{\theta}\left(\boldsymbol{z}^{(j)}|\mathcal{E}, \boldsymbol{x}, \boldsymbol{z}^{(<j)}\right)$ and $\boldsymbol{z}^{(0)}$ is a null string.

% \textcolor{red}{Here, a set of examples $\mathcal{E} = \left\{\left(q_i, a_i, \mathcal{Z}_i \right) \right\}_{i=1}^{\lvert \mathcal{E} \rvert}$ includes the reasoning paths $\mathcal{Z}_i$ for each question $q_i$.}
Since marginalizing over all possible reasoning paths $\mathcal{Z}$ is intractable, most prompting methods approximate it by sampling them as follows:
\begin{equation}
\begin{split}
    &\hat{\boldsymbol{y}} =  \underset{\boldsymbol{y}}{\arg\!\max}\ \ p_{\theta}\left(\boldsymbol{y} | \mathcal{E}, \boldsymbol{x}, \mathcal{Z'}\right),\\
    &\mbox{where } \mathcal{Z'} = f\left(\mathcal{Z} | \mathcal{E}, \boldsymbol{x}  \right),
\end{split}
\end{equation}
where the function $f$ is the function to generate the reasoning path for obtaining the optimal answer.
The CoT prompting~\cite{wei2022chain} generates the most probable reasoning path and the answer with the function $f\left(\mathcal{Z} | \mathcal{E}, \boldsymbol{x}  \right) = \underset{\mathcal{Z}}{\text{arg}\max}\ p_\theta(\mathcal{Z}| \mathcal{E}, \boldsymbol{x})$.
% where $p_\theta(\mathcal{Z}| \mathcal{E}, \boldsymbol{x}) =% \prod_{i=2}^m p_\theta(\boldsymbol{z}^{(i)} | \boldsymbol{z}^{(<i)}, \mathcal{E}, \boldsymbol{x})p_\theta(\boldsymbol{z}^{(1)} | \mathcal{E}, \boldsymbol{x})$.
% \prod_{j=1}^m p_\theta(\boldsymbol{z}^{(j)} | \boldsymbol{z}^{(<j)}, \mathcal{E}, \boldsymbol{x})$. 
% Self-consistency
% So, the decomposable reasoning paths are produced sequentially without decomposition and verification.



% $\boldsymbol{y} \sim p_{\theta}^{CoT}\left(\boldsymbol{y} | \mathcal{E}, \boldsymbol{x}, \boldsymbol{z}^{(1)}, \dots, \boldsymbol{z}^{(m)} \right)$.
% In sum, CoT prompting generates an answer along with intermediate reasoning steps $\left[\boldsymbol{y}, \boldsymbol{z}^{(i)}, \dots ,\boldsymbol{z}^{(m)} \right] \sim p_{\theta}^{CoT}\left(\boldsymbol{y}, \boldsymbol{z}^{(i)} \dots \boldsymbol{z}^{(m)} | \boldsymbol{x} \right)$ without the verification of the rationality of the reasoning steps~\textcolor{red}{[CITE]}.

==> Tables_Figures_tex/gpt_main_table.tex <==
% {\renewcommand{\arraystretch}{1.35}%
\begin{table*}[!ht]
    \small
    % \setlength{\tabcolsep}{0pt} 
    
    % \begin{tabular}{l|C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}|C{1.3cm}C{1.3cm}C{1.3cm}|C{1.3cm}}
    \centering
    % \resizebox{\textwidth}{!}{
    \begin{tabular}{l|cccc|cc|c}
        \toprule
          Datasets& \multicolumn{4}{c|}{2WikiMultihopQA}&\multicolumn{2}{c|}{MusiQue} & \multicolumn{1}{c}{Bamboogle}\\
          Metrics & EM & F1 & Prec. & Recall & EM & F1 & EM  \\
         \midrule 
         \midrule
         No retrieval&33.4 & 41.10 & 40.62 & 42.51 & 8.2	& 17.71 & 44.0 \\
         One retrieval & 50.6 & 61.33 & 60.55 & 62.23 & 17.2 & 27.66 & 58.4\\
         Verify-and-Edit &  50.0 & 61.01 & 61.15 & 61.86  & 18.6	& 28.57 & 56.0\\
         FLARE & 51.0 & 61.53 & 60.31 & 62.61 & 18.4	& 28.68 & 55.2\\
         IRCoT & 51.4	 & 61.87 & 61.32 & 62.57  & 20.6 & 29.94 & 59.2 \\         
         \midrule
         Graph-guided reasoning & \textbf{52.4} & \textbf{62.78} & \textbf{62.68} & \textbf{63.48} & \textbf{22.0} & \textbf{31.98} & \textbf{63.2}\\
        \bottomrule
    \end{tabular}
    \vspace{-2mm}
    \caption{Performance comparison on multi-hop question answering datasets with GPT 3.5 model in the open-book setting. \textbf{Bold} indicates the best performance. 
    % The baselines results are reported from \cite{kang2022knowledge}.
    }
    % \vspace{-5mm}
    \label{tab:gpt}
    % }
\end{table*}
% }

==> Tables_Figures_tex/graph_fig.tex <==
\begin{figure}[t] 
\centering
\includegraphics[width=0.99\columnwidth]{Figures/graph_Fig3.png}
\vspace{-2mm}
\caption{
Graphs generated by graph construction prompting.
}
\label{fig:graph_fig}
\end{figure}

% The Knowledge path Prompting-based Dialogue Generation~(KPDG) model generates responses with a Knowledge Graph~(KG).
% Given a dialog history, multi{\textendash}hop knowledge paths are retrieved from the KG.
% Then, soft prompts are added to knowledge paths to improve path embeddings~\ref{sec:4.1}.
% We retrieve context{\textendash}relevant knowledge paths by calculating the relevance between the path embeddings and a context embedding~\ref{sec:4.2}.
% Finally, we generate responses with dialogue history and the retrieved knowledge paths~\ref{sec:4.3}.


==> Tables_Figures_tex/qual_bak.tex <==

\begin{table}[!t]
    \small
    % \setlength{\tabcolsep}{0pt} 
    
    % \begin{tabular}{l|C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}|C{1.3cm}C{1.3cm}C{1.3cm}|C{1.3cm}}

    \centering
    % \resizebox{\textwidth}{!}{
    \begin{tabular}{l}
        \toprule
          \textbf{Question: }Where did the performer of song How Can\\I Tell Her It's Over die?\\
          \textbf{Ground Truth: } Branson, Missouri\\
          % Metrics & EM & F1 & Prec. & Recall \\
         % \midrule 
         \midrule
         \textbf{w/o graph guidance:}\\
         The performer of the song How Can I Tell Her It's Over,\\ died on September 25, 2012.\\
         So the answer is September 25, 2012.\\
         \midrule
         \textbf{with graph guidance: }\\
         (1) Who performed the song How Can I Tell Her\\It's Over?\\
         \textcolor{gray}{\tiny('How Can I Tell Her It'S Over', performer, x)}\\
         The song How Can I Tell Her It's Over was performed by\\ Andy Williams.\\
         (2) Where did Andy Williams die?\\
         \textcolor{gray}{\tiny(`Andy Williams', death place, y)}\\
         Andy Williams died in Branson, Missouri.\\
         So the answer is Branson, Missouri.\\
        \midrule
        \midrule
          \textbf{Question: }Who is the paternal grandfather of Beatrice I,\\Abbess Of Quedlinburg?\\
          \textbf{Ground Truth: } Conrad II\\
          % Metrics & EM & F1 & Prec. & Recall \\
         \midrule
         \textbf{w/o graph guidance:}\\
        Beatrice I, Abbess Of Quedlinburg's paternal grandfather\\is Henry III, Holy Roman Emperor.
        \\So the answer is Henry III, Holy Roman Emperor.\\
         \midrule
         \textbf{with graph guidance: }\\
         (1) Who is Beatrice I, Abbess Of Quedlinburg's father?\\
         \textcolor{gray}{\tiny(`Beatrice I, Abbess Of Quedlinburg', father, x)}\\
         Beatrice I, Abbess Of Quedlinburg's father is Henry III.\\ 
         (2) Who is Henry III's father?\\
         \textcolor{gray}{\tiny(`Henry III', father, y)}\\
         Henry III's father is Conrad II.\\ 
         So the answer is Conrad II.\\

        \bottomrule
    \end{tabular}
    \vspace{-2mm}
    \caption{Comparison on reasoning steps and answers generated by prompting without and with the graph guidance.
    % The baselines results are reported from \cite{kang2022knowledge}.
    }
    \label{tab:qual}
    \vspace{-5mm}
    % }
\end{table}

%          
% Answer: 



==> Tables_Figures_tex/ret_main_table.tex <==
% {\renewcommand{\arraystretch}{1.35}%
\begin{table*}[!ht]
% \jk{Put retrival result tables before non-retrival ones. Also, add GPT result tables.}
    \small
    % \setlength{\tabcolsep}{0pt} 
    
    % \begin{tabular}{l|C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}|C{1.3cm}C{1.3cm}C{1.3cm}|C{1.3cm}}
    \centering
    % \resizebox{\textwidth}{!}{
    \begin{tabular}{l|cc|cc|c|cc|cc|c}
        \toprule
          Models & \multicolumn{5}{c|}{Llama2-13b-chat} & \multicolumn{5}{c}{Llama2-70b-chat} \\
          \midrule
          Datasets& \multicolumn{2}{c|}{2WikiQA}&\multicolumn{2}{c|}{MusiQue} & \multicolumn{1}{c|}{Bamboogle}& \multicolumn{2}{c|}{2WikiQA}&\multicolumn{2}{c|}{MusiQue} & \multicolumn{1}{c}{Bamboogle}\\
          Metrics    & EM & F1     & EM & F1 & EM  & EM & F1     & EM & F1 & EM  \\
         \midrule 
         \midrule
         No retrieval&29.4 & 33.12 & 7.4 & 15.27 & 44.0 &35.2 & 41.38 & 13.4 & 22.95 & 47.2\\
         One retrieval & 44.8 & 52.32  & 15.2 & 24.85 & 53.4& 52.8 & 61.98 &  24.4 & 35.41 & 57.6\\
         Verify-and-Edit &  47.0 & 55.05   & 19.2 & 28.27 & 55.2 &  53.4 & 62.87  & 25.2 & 37.65 & 60.8 \\
         FLARE & 46.2 & 55.10  & 18.6 & 27.61 & 56.8 & 53.8 & 62.95  & 26.0 & 38.87 & 60.8\\
         IRCoT &  48.2 & 55.62  & 20.4 & 28.84 & 57.6 &  53.8 & 63.14 &  26.6 & 39.56 & 60.0 \\         
         \midrule
         Graph-guided reasoning & \textbf{50.0} & \textbf{56.93}  & \textbf{21.8} & \textbf{31.24} & \textbf{59.2} & \textbf{58.4} & \textbf{63.30} &  \textbf{28.4} & \textbf{40.37} & \textbf{64.0}\\
        \bottomrule
    \end{tabular}
    \vspace{-2mm}
    \caption{Performance comparison on multi-hop question answering datasets with Llama-2-13b-chat and Llama-2-70b-chat model in the open-book setting. \textbf{Bold} indicates the best performance. 
    % The baselines results are reported from \cite{kang2022knowledge}.
    }
    \label{tab:ret}
    \vspace{-2mm}
    % }
\end{table*}
% }

==> Tables_Figures_tex/temp_tab.tex <==
% {\renewcommand{\arraystretch}{1.35}%
\begin{table*}[!ht]
    \small
    % \setlength{\tabcolsep}{0pt} 
    
    % \begin{tabular}{l|C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}|C{1.3cm}C{1.3cm}C{1.3cm}|C{1.3cm}}
    \caption{Performance comparison on multi-hop question answering datasets with Llama-2-70b model. \textbf{Bold} indicates the best performance. 
    % The baselines results are reported from \cite{kang2022knowledge}.
    }
    \label{tab:table1}
    \centering
    % \resizebox{\textwidth}{!}{
    \begin{tabular}{l|cccc|cc|c}
        \toprule
          Datasets& \multicolumn{4}{c|}{2WikiMultihopQA}&\multicolumn{2}{c|}{MusiQue} & \multicolumn{1}{c}{Bamboogle}\\
          Metrics & EM & F1 & Prec. & Recall & EM & F1 & EM  \\
         \midrule 
         \midrule
         Chain-of-Thoughts&35.2 & 41.38 & 41.28 & 42.17 & 13.4 & 22.95 & 48.6 \\
         Zero-Plus-Few-Shot CoT & 35.8 & 42.61 & 42.47 & 43.43 & 14.4 & 23.24 & 49.6\\
         Self-Consistency & 37.6 & 44.04 & 43.98 & 44.99  & 14.8 & 23.85 & 50.2\\
         Self-ask & 37.8 & 44.38 & 44.26 &45.39 & 13.4 & 24.15 & 49.8\\
         \midrule
         Graph-guided reasoning & \textbf{39.2} & \textbf{46.87} & \textbf{45.98} & \textbf{47.52} & \textbf{15.2} & \textbf{25.17} & \textbf{52.0}\\
        \bottomrule
    \end{tabular}
    % }
\end{table*}
% }

==> Tables_Figures_tex/temp_tab2.tex <==
% {\renewcommand{\arraystretch}{1.35}%
\begin{table*}[!ht]\jk{Put retrival result tables before non-retrival ones. Also, add GPT result tables.}
    \small
    % \setlength{\tabcolsep}{0pt} 
    
    % \begin{tabular}{l|C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}|C{1.3cm}C{1.3cm}C{1.3cm}|C{1.3cm}}
    \caption{Performance comparison on multi-hop question answering datasets with Llama-2-70b model in the open-book setting. \textbf{Bold} indicates the best performance. 
    % The baselines results are reported from \cite{kang2022knowledge}.
    }
    \label{tab:table2}
    \centering
    % \resizebox{\textwidth}{!}{
    \begin{tabular}{l|cccc|cc|c}
        \toprule
          Datasets& \multicolumn{4}{c|}{2WikiMultihopQA}&\multicolumn{2}{c|}{MusiQue} & \multicolumn{1}{c}{Bamboogle}\\
          Metrics & EM & F1 & Prec. & Recall & EM & F1 & EM  \\
         \midrule 
         \midrule
         No retrieval&35.2 & 41.38 & 41.28 & 42.17 & 13.4 & 22.95 & 48.6 \\
         One retrieval & 52.8 & 61.98 & 61.9 & 62.32 & 24.4 & 35.41 & 58.8\\
         Verify-and-Edit &  53.4 & 62.87 & 62.56 & 63.98  & 25.2 & 37.65 & 60.0 \\
         FLARE & 53.8 & 62.95 & 63.32 &64.05 & 26.0 & 38.87 & 61.2\\
         IRCoT &  53.8 & 63.14 & 63.43 & 64.48  & 26.6 & 39.56 & 62.0 \\         
         \midrule
         Graph-guided reasoning & \textbf{54.2} & \textbf{63.97} & \textbf{63.7} & \textbf{65.54} & \textbf{27.6} & \textbf{40.12} & \textbf{62.8}\\
        \bottomrule
    \end{tabular}
    % }
\end{table*}
% }

==> Tables_Figures_tex/temp_tab3.tex <==
% {\renewcommand{\arraystretch}{1.35}%
\begin{table*}[!ht]
    \small
    % \setlength{\tabcolsep}{0pt} 
    
    % \begin{tabular}{l|C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}|C{1.3cm}C{1.3cm}C{1.3cm}|C{1.3cm}}
    \caption{Performance comparison on multi-hop question answering datasets with Llama-2-13b model. \textbf{Bold} indicates the best performance. 
    % The baselines results are reported from \cite{kang2022knowledge}.
    }
    \label{tab:table3}
    \centering
    % \resizebox{\textwidth}{!}{
    \begin{tabular}{l|cccc|cc|c}
        \toprule
          Datasets& \multicolumn{4}{c|}{2WikiMultihopQA}&\multicolumn{2}{c|}{MusiQue} & \multicolumn{1}{c}{Bamboogle}\\
          Metrics & EM & F1 & Prec. & Recall & EM & F1 & EM  \\
         \midrule 
         \midrule
         Chain-of-Thoughts&29.4 & 33.12 & 33.26 & 33.48 & 7.4 & 15.27 & 44.4 \\
         Zero-Plus-Few-Shot CoT & 30.4 & 33.88 & 33.93 & 34.14 & 7.4 & 15.62 & 45.4\\
         Self-Consistency & 31.8 & 37.87 & 38.55 & 38.88  & 8.2 & 16.25 & 46.6\\
         Self-ask & 32.0 & 38.23 & 38.65 &38.62 & 7.8 & 15.77 & 46.2\\
         \midrule
         Graph-guided reasoning & \textbf{34.6} & \textbf{41.52} & \textbf{41.25} & \textbf{42.03} & \textbf{11.2} & \textbf{20.31} & \textbf{47.4}\\
        \bottomrule
    \end{tabular}
    % }
\end{table*}
% }

==> Tables_Figures_tex/temp_tab5.tex <==
% {\renewcommand{\arraystretch}{1.35}%
\begin{table*}[!ht]
    \small
    % \setlength{\tabcolsep}{0pt} 
    
    % \begin{tabular}{l|C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}|C{1.3cm}C{1.3cm}C{1.3cm}|C{1.3cm}}
    \caption{Performance comparison on multi-hop question answering datasets with Llama-2-13b model in the open-book setting. \textbf{Bold} indicates the best performance. 
    % The baselines results are reported from \cite{kang2022knowledge}.
    }
    \label{tab:table5}
    \centering
    % \resizebox{\textwidth}{!}{
    \begin{tabular}{l|cccc|cc|c}
        \toprule
          Datasets& \multicolumn{4}{c|}{2WikiMultihopQA}&\multicolumn{2}{c|}{MusiQue} & \multicolumn{1}{c}{Bamboogle}\\
          Metrics & EM & F1 & Prec. & Recall & EM & F1 & EM  \\
         \midrule 
         \midrule
         No retrieval&29.4 & 33.12 & 33.26 & 33.48 & 7.4 & 15.27 & 44.4 \\
         One retrieval & 44.8 & 52.32 & 52.85 & 52.84 & 15.2 & 24.85 & 55.2\\
         Verify-and-Edit & 47.0 & 55.05 & 55.84 & 56.13  & 19.2 & 28.27 & 57.6\\
         FLARE & 46.2 & 55.10 & 55.47 & 56.15 & 18.6 & 27.61 & 58.4\\
         IRCoT & 48.2 & 55.62 & 57.10 & 56.45  & 20.4 & 28.84 & 58.6\\         
         \midrule
         Graph-guided reasoning & \textbf{48.8} & \textbf{56.13} & \textbf{57.72} & \textbf{56.54} & \textbf{21.2} & \textbf{30.9} & \textbf{59.2}\\
        \bottomrule
    \end{tabular}
    % }
\end{table*}
% }
